Beating $(1-1/e)$-Approximation for Weighted Stochastic Matching

In the stochastic weighted matching problem, the goal is to find a large-weight matching of a graph when we are uncertain about the existence of its edges. In particular, each edge $e$ has a known weight $w_e$ but is realized independently with some probability $p_e$. The algorithm may query an edge to see whether it is realized. We consider the well-studied query commit version of the problem, in which any queried edge that happens to be realized must be included in the solution. Gamlath, Kale, and Svensson showed that when the input graph is bipartite, the problem admits a $(1-1/e)$-approximation. In this paper, we give an algorithm that for an absolute constant $\delta > 0.0014$ obtains a $(1-1/e+\delta)$-approximation, therefore breaking this prevalent bound.

==> overview.tex <==
%\section{The Linear Program}
%In this section, we describe our algorithm which consists of two parts. The first parts is an LP which gives an upper-bound on the optimal solution of the problem. We then design a rounding procedure which given a solution of this LP, decides which edges to query and in which order. The LP which we barrow from~\cite{DBLP:conf/soda/GamlathKS19} is as follows.
%
%%\begin{align*}
%%\max_{\mathbf{x}} \qquad &\sum_{e\in E} x_e	\,,& \\
%%\textrm{s.t.} \qquad & \sum_{e \in F} x_e \le \Pr[\text{an edge in $F$ exists}]& \forall u \in A \cup B,  \forall F \subseteq E_u \,, \\
%%&x_e \ge 0& \forall e \in E \,. 
%%\end{align*}
%\vspace{5mm}
%\newlength{\LPlhbox}
%\settowidth{\LPlhbox}{(LP-Match)}%
%\noindent%
%\parbox{\LPlhbox}{\begin{align}
%               \tag{LP-Match}\label{LP-Match}
%         \end{align}}%
%\hspace*{\fill}%
%\begin{minipage}{\linewidth-2cm}
% \begin{align}
%\nonumber \max_{\mathbf{x}} \qquad &\b{x} \cdot \b{w}	\,& \\
%\textrm{s.t.} \qquad & \sum_{e \in F} x_e \le \Pr[\text{an edge in $F$ exists}]& \forall u \in A \cup B,  \forall F \subseteq E_u  \\
%&x_e \ge 0& \forall e \in E 
%\end{align}
%\end{minipage}
%\vspace{5mm}
%
%In the LP above $E_u$ is the set of adjacent edges of vertex $u$ and $x_e$ is the probability that $e$ is part of the optimal solution. For a vertex $u$ and any subset $F \subseteq E_u$,  $\sum_{e \in F} x_e$ is the probability that at one of the edges in $F$ are in the optimal solution. Hence,  $\sum_{e \in F} x_e$ should be bounded by the probability that at least one of the edges in $F$ exists. Since each edge  $e\in F$ exists independently with probability $p_e$, we have $\Pr[\text{an edge in $F$ exists}] = 1- \prod_{e \in F} (1-p_e)$. 
%
%\begin{lemma}[\cite{DBLP:conf/soda/GamlathKS19}]
%	The optimal solution of \ref{LP-Match} is an upper-bound for \opt. Moreover, this solution can be found in polynomial time.
%\end{lemma}
%
%A nice property of this LP which is crucial for the $(1-1/e)$-approximation algorithm of Galamth~\etal{} is as follows. For any vertex $v$, it is possible to randomly permute its edges such that for any edge $e$ the probability of it being the first realized edge in the permutation is no smaller than $x_e$. To make this an exact equality, sometimes this permutations needs to be over a subset of $E_v$ instead of the whole set. The formal statement of this property is provided in the below lemma.
%
%\begin{lemma}[\cite{DBLP:conf/soda/GamlathKS19}]\label{lemma:dist}
%	Let {\b x} be a solution of \ref{LP-Match} (non necessarily the optimal solution). For any vertex $v$, there exists a distribution $\mathcal{D}^{\b x}_v$ over permutations of subsets of $E_v$, such that for any edge $e\in N_v$ the probability that $e$ is outputted by the following algorithm is exactly equal to $x_e$
%	
%	\end{lemma}
%
%
%\begin{tboxalg2e}{}
%\begin{algorithm}[H]
%% \caption{Vertex and pair oracles.}
%% \label{alg:edgeoracle}
%% \caption{``vertex oracle''}	
%    \DontPrintSemicolon
%        Let $\pi_v\sim \mathcal{D}^{\b x}_v$.\;
%        \ForEach{$e$ permuted in the order of  $\pi_v$}{
%        Examine edge e.\;
%        \If{$e$ is realized}
%        {Output $e$ and end the algorithm.}
%        }
%\end{algorithm}
%\end{tboxalg2e}


%\section{The Rounding Procedure}
%
%Our rounding procedure consists of two parts. First is an algorithm which outputs a $(1-1/e)$ approximate matching and has some new desired properties. We will refer to this al \algone. The second part is using \algone{} in order to design  another rounding procedure with approximation ratio higher than $(1-1/e)$. 
%
%
%Before presenting \algone, we first explain a a simplified version of it which outputs a $(1-1/e)$ approximate matching for unweighted graphs. (This is also a simplified version of \GKS.) Let us start by providing a definition which we will use in the rest of the paper.
%
%\begin{definition}[Examining an edge $e$]
%We examine an edge to determine whether it is realized or not. If both its end-points are unmatched, examining $e$ is equivalent to querying it. It is always guaranteed that in this case, $e$ joins the matching if it is realized. 
%  
%At some points in our algorithm we also need to use the information about realization of an edge who has at least one matched end-point. In this scenario, we cannot query the edge because it cannot join the matching. Instead, we just toss a coin which with probability $p_e$ decides that the edge is realized. In such cases, it is guaranteed the edge will not join the matching if realized. 
%\end{definition}
%
%\SetKwFunction{SPM}{SimpleMatching}
%
%\paragraph{The simplified algorithm.} This algorithm is stated formally in as \SPM  below. In this algorithm, we first draw a permutation $\pi$ over vertices in $A$ uniformly at random. Going over $A$ in this order, for any vertex $v\in A$, we draw a permutation $\pi_v$ over its edges from $\mathcal{D}^{\b x}_v$ (defined in Lemma~\ref{lemma:dist}). We then examine edges of $A$ in this order and stop when one of them is realized. Let us denote this edge by $e=(v,u)$. Vertex $v$ then sends a proposal to $u$. If $u$ is unmatched, it accepts the proposal and $e$ joins the matching. If $u$ is already matched, it rejects the proposal and $v$ remains unmatched forever. The algorithm then proceeds to repeat this for the next edge in permutation $\pi$. 
%
%
%\begin{tboxalg2e}{}
%\begin{algorithm}[H]\label{alg:simple}
%% \caption{Vertex and pair oracles.}
%% \label{alg:edgeoracle}
%% \caption{``vertex oracle''}
%    \SetKwProg{Fn}{Function}{:}{}	
%    \DontPrintSemicolon
%    \Fn{\SPM{$G=(A, B, E), \b x$}}{
%    Let $M=\emptyset$ be a matching of $E$.\;
%    Let $\pi$ be a permutation over vertices in $A$ chosen uniformly at random. \;
%    Mark all the vertices as alive.\;
%\ForEach {$v$ in the order of $\pi$}{
%        Let $\pi_v\sim \mathcal{D}^{\b x}_v$.\;
%        \ForEach{$e=(v,u)$ permuted in the order of  $\pi_v$}{
%        Examine edge $e$.\\
%        \If{$e$ is realized}{ Vertex $v$ sends a proposal to $u$.\\
%        If $u$ is unmatched, it accepts the proposal and $e$ joins the matching.\\
%        Terminate the loop.}
%        }
%        }
%        \Return $M$.
%        }
%\end{algorithm}
%\end{tboxalg2e}
%\vspace{4 mm}
%
%
%We claim that \SPM{$G, \b x$} matches any vertex $u\in B$  with probability at least $$(1-1/e)\sum_{e\in E_u} x_e.$$ If we consider unweighted graphs, this implies a lower-bound of $(1-1/e)$ for the approximation ratio. Observe that this algorithm matches vertex $u$ if it receives at least one proposal from its neighbors. Since $\pi_v$ is drawn from $\mathcal{D}^{\b x}_v$, by Lemma~\ref{lemma:dist}, the probability of $u$ receiving a proposal from any neighbor $v$ is exactly $x_{(v,u)}$. Combining this with the fact that any vertex $v\in A$ sends its proposals independently of other vertices in $A$, we can write:
%
%
%\begin{align*}\Pr[u \text{ is matched }] &= \Pr[u \text{ receives at least one proposal}]\\
%& \geq  (1-1/e)\sum_{e\in E_u} x_e \hspace{45 mm} \text{ (due to Fact~\ref{fact1} stated below)}\\
%\end{align*} 
%
%
% \begin{fact}\label{fact1}
% Let $x_1, \dots, x_k$ be a set of independent Bernoulli random variables with  $\E[X]\leq 0$, where $X$ is their sum. We have $$\Pr\left[X > 0\right] \geq 1-e^{-\E[X]}\geq \E[X](1-1/e).$$
% \end{fact}
% 
% 
% As mentioned before, this is also a simplified version of \GKS. To make this algorithm work for weighted graphs, they allow each vertex $u\in B$ to decide which proposal it is going to accept instead of just accepting the first one. To make this decision, for each vertex $u$ they run an algorithm similar to the one designed for the prophet secretary problem by \mdcomment{verify} which results in 
% $$\sum_{e\in E_u}\Pr[e \text{ joins the matching}].w_e \geq (1-1/e) x_ew_e,$$ for any vertex $u\in B,$
% and thus a $(1-1/e)$ approximation algorithm. Let us emphasize that this is a rephrased version of their algorithm for the sake of comparison with ours. Of course, to describe their algorithm using our language, we need to change what examining an edge means, but we will not go into more details here.
% 
% Now, let us explain the desired properties that we are trying to achieve by designing a new $(1-1/e)$-approximate matching. Define $\ubar=\max_{u\in B} \sum_{e\in E_u} x_e.$ These properties as follows.
% 
% \begin{enumerate}
% \item We want \algone{} to match any edge with probability at least $(1-1/e)x_e$. This property is not satisfied by either \SPM or \GKS. For instance, in \GKS{} if an edge has a very low weight, it may have a very small of joining the matching. This property directly implies that \algone{} is a $(1-1/e)$ approximation algorithm.
%\item Finally we want the probability of the edges being matched to be an increasing function of $\ubar$. In the other words, if  $\ubar$ is smaller than one by a constant, we want \algone{} to match any edge with probability at least $(1-1/e+c)x_e$, where $c$ is a constant. This implies that in this scenario, \algone{} itself achieves approximation ratio larger than $(1-1/e)$.
% \item We also want each edge to remain unmatched with a large enough probability, that is a constant fraction of $x_e$. This property allows us to show that for some instances of the problem, running \algone{} twice gives us an improved algorithm. That is we once run \algone{} on $G$ and once on the edges that are not queried and have unmatched end-points in the first run.
% \end{enumerate}

 

%
%\section{The Analysis}
%\begin{lemma}
%\label{lem:prm1}
%
%For any edge $e$, we have the following.
%\begin{align*}
%\frac{(1-e^{-\ubar})x_e}{\ubar} \le \Pr[e \in \match_1] \le \frac{x_e(1+e^{-\ubar})}{2}.
%\end{align*}
%\end{lemma}
%
%\begin{proof}
%Consider Algorithm~\ref{alg} which we use to construct $\match_1$.
%Note that in this algorithm, we use dummy edges to ensure that for any vertex $u\in B$, we have $x_u \gets \sum_{e\in E', e \ni u} x_e =\ubar.$  Suppose that $e=(v,u)$. We claim that $\Pr[e \in \match_1]$ is minimized when  except $e$, $u$ has a large number of edges (approaching $\infty$) with the total contribution of $\ubar-x_e$. On the other hand, it is maximized  when $u$ is only incident to one other edge with the contribution of $1-x_e$. To prove our claim, we take an edge $e'=(v', u)\neq e$ and show that replacing it with two edges $e_1'$ and $e_2'$ with $x_{e_1'}=x_{e_2'}= x_e/2$ increases $\Pr[e \in \match_1]$.
%
%Let $\pi$ be the permutation over vertices in $A'$ chosen uniformly at random in the algorithm constructing $\match_1$. For any edge $(v'', u)\in E'$, let $s_v''$ be a Bernoulli random variable which is equal to one if $v''$ is the first vertex from set $B/\{v'\}$ to send a proposal to $u$. This implies that edge $e$ only has a chance of joining the matching only if $s_v=1$. In addition to that $v'$ should not send a proposal before $v$.  Thus, we have 
%
%\begin{align*}
% \Pr[e \in \match_1] &=  \Pr\left[v' \text{ does not send a proposal to } u \text{ before } v \mid s_v=1\right]\Pr[s_v=1] \\
% & = \left(1- \Pr\left[\pi(v') < \pi(v)s \mid s_v=1\right]\Pr\left[v' \text{sends a proposal} \mid s_v=1\right]\right)\Pr[s_v=1] \\
% & = (1- 0.5\cdot \tilde{x}_{e'})\Pr[s_v=1].
%\end{align*}
%Now if we replace $e'$ with $e_1'=(v'_1, u)$ and $e_2' = (v'_2, u)$ we get 
%
%
%
%\begin{align*}
% \Pr[e \in \match_1] &=  \Pr\left[\text{neither } v_1'  \text{ nor }  v_2' \text{ send a proposal to } u \text{ before } v \mid s_v=1\right]\Pr[s_v=1] \\
% & = (1- 0.5\cdot \tilde{x}_{e_1'} - 0.5\cdot \tilde{x}_{e_2'} + 0.25\cdot \tilde{x}_{e_1'}\tilde{x}_{e_2'})\Pr[s_v=1].
%\end{align*}
%To prove our claim, we need to show 
%\begin{align*}
%(1- 0.5\cdot \tilde{x}_{e_1'} - 0.5\cdot \tilde{x}_{e_2'} + 0.25\cdot \tilde{x}_{e_1'}\tilde{x}_{e_2'})\Pr[s_v=1]- (1- 0.5\cdot \tilde{x}_{e'})\Pr[s_v=1] \leq 0.	
%\end{align*}
%Since $\Pr[s_v=1]$ is a non-negative number, we can factor  $0.5\cdot\Pr[s_v=1]$ out and get
%
%\begin{align*}
%- \tilde{x}_{e_1'} -  \tilde{x}_{e_2'} + 0.5\cdot \tilde{x}_{e_1'}\tilde{x}_{e_2'} +  \tilde{x}_{e'} \leq 0.	
%\end{align*}
%Now, plugging in the values of $\tilde{x}_{e'}$, $\tilde{x}_{e_1'}$, and $\tilde{x}_{e_2'}$, we need to prove that the following term is not positive for any $\ubar\in [0,1]$ and $x_e\in [0,\ubar]$.
%
%
%\begin{align*}
%	-2\frac{(e^\ubar-1)(\ubar  -x_e/2) x_e/2}{\ubar (e^\ubar- e^{x_e/2}) }+ 0.5\left(\frac{(e^\ubar-1)(\ubar  -x_e/2) x_e/2}{\ubar (e^\ubar- e^{x_e/2}) }\right)^2 +\frac{(e^\ubar-1)(\ubar  -x_e) x_e}{\ubar (e^\ubar- e^{x_e})}.
%\end{align*}
%After factoring out $\frac{(e^\ubar-1) x_e}{8\ubar}$ (which is always positive) from all terms, it suffices to prove: 
%
%\begin{align*}
%	-\frac{8(\ubar  -x_e/2)}{ (e^\ubar- e^{x_e/2}) }+ \frac{(e^\ubar-1)(\ubar  -x_e/2)^2 x_e}{\ubar (e^\ubar- e^{x_e/2})^2 } +\frac{8(\ubar  -x_e)}{ (e^\ubar- e^{x_e})}\leq 0.
%\end{align*}
%We do so by plotting this function and observing that it is not positive for any $\ubar\in [0,1]$ and $x_e\in [0,\ubar]$. 
%This proves our claim that $\Pr[e \in \match_1]$ is minimized when except $e$, $u$ has a large number of edges (approaching $\infty$) with the total contribution of $\ubar-x_e$. On the other hand, it is maximized  when $u$ is only incident to one other edge with the contribution of $1-x_e$. Now, we are ready to prove the desired lower and upper bounds for $\Pr[e \in \match_1]$. We start by proving the lower-bound.\\
%\\
%\textbf{Lower-bound:}
%\\
%Let $k$ denote the number of vertices adjacent to $u$ other than $v$ and define $\delta=\ubar-x_e$. We already proved that $\Pr[e \in \match_1]$ is minimized when $k\rightarrow \infty$ and $x_e' = \delta/k$  for any $e'\neq e$. Thus,
%\begin{align*}\Pr[e \in \match_1] &= \Pr[e \text{ is proposed}]\sum_{i=0}^k\Pr[\text{There are } i \text{ edges before } e \text{ in  } \pi \wedge \text{none of them are proposed}]
%\\&\geq g(x_e)\times \lim_{k\rightarrow \infty}\left(\sum_{i=0}^{k}\frac{1}{k+1} \left(1-g\left(\delta/k\right)^i\right)\right) 
%\\& = \frac{g(x_e)}{k}\times \sum_{i=0}^{k} \left(1-\left( \delta/k \right)^i\right) 
%\\&= g(x_e)\times  \sum_{i=0}^{k} \frac{e^{-i\delta/k}}{k} , \end{align*}
%where the third equality is due to $\lim_{x\rightarrow 0}g(x)= x$.
%Since $k\rightarrow \infty$, we can replace the above summation with an integration as follows:
%$$\sum_{i=0}^{k} \frac{e^{-i\delta/k}}{k}=\int_{0}^{1} e^{-y\delta} dy= \frac{1-e^{-\delta}}{\delta} = \frac{1-e^{-\ubar + x_e}}{\ubar - x_e}. $$
%This gives us:
%\begin{align*} \Pr[e \in \match_1]& \geq \frac{(e^\ubar-1)(\ubar  -x_e) x_e}{\ubar (e^\ubar- e^{x_e})}\times \frac{1-e^{-\ubar + x_e}}{\ubar - x_e}
%\\ &= \frac{x_e}{\ubar}\times \frac{(e^\ubar-1)(1-e^{-\ubar + x_e})}{e^\ubar-e^{x_e}}
%\\ &=\frac{x_e}{\ubar}\times \frac{e^\ubar  - e^{x_e}-1 +  e^{-\ubar + x_e}}{e^\ubar-e^{x_e}}	
%\\ &=\frac{x_e}{\ubar}\times \frac{(e^\ubar - e^{x_e}) (1-e^{-\ubar})}{e^\ubar-e^{x_e}}	
%\\ &=\frac{x_e(1-e^{-\ubar})}{\ubar}
%\end{align*}
% This completes the proof of our desired lower-bound. \\
% \\
% \textbf{Upper-bound:}\\
% Now, we proceed to prove the following upper-bound:
%$$\Pr[e \in \match_1] \le \frac{1}{2}(1 + e^\ubar) x_e.$$ 
%Recall that we have already proved that this probability is maximized  when $u$ is only incident to one other edge $e'$ with  $x_{e'}=1-x_e$. Hence, we have 
%\begin{align*}\Pr\left[e \in \match_1\right] &= \Pr[e \text{ is proposed}]\left(\Pr[\pi(e) < \pi(e') ] + \Pr[\pi(e) > \pi(e')  \wedge e' \text{ is not proposed}]\right)
%\\ & = g(x_e) \left( 0.5 + 0.5(1-g(x_{e'})\right)
%\\& = g(x_e) \left( 1-0.5g(x_{e'})\right)
%\end{align*}
%Note that $g(x)/x=\frac{(e^\ubar-1)(\ubar  -x)}{\ubar (e^\ubar- e^x)}$ is a decreasing function of $x$. As such, 
%$$g(x_e)/x_e\leq \lim_{x_e\rightarrow 0}(g(x_e)/x_e) \leq 1,$$ and 
%$$g(x_{e'})/x_{e'}\geq \lim_{x_{e'}\rightarrow \ubar}(g(x_{e'})/x_{e'}) \geq (1 - e^{-\ubar})/\ubar.$$
%As a result, we have 
%\begin{align*}\Pr\left[e \in \match_1\right] &= g(x_e) \left( 1-0.5g(x_{e'})\right)
%\\& \leq x_e (1-0.5x_{e'}(1 - e^{-\ubar})/\ubar)
%\\& \leq x_e (1-0.5(\ubar-x_e)(1 - e^{-\ubar})/\ubar)
%\\& \leq x_e (1-0.5(1 - e^{-\ubar}))
%\\& \leq x_e (0.5+0.5e^{-\ubar})
%\\& \leq \frac{x_e}{2}(1+e^{-\ubar}).
%\end{align*}
%This proves our desired upper-bound and completes the proof of this lemma.
%\end{proof}
%
%
%
%
%\input{nextround}

==> proof.tex <==
%\begin{lemma}
%Consider an edge $e=(v,u)$ that is available at the round $i$ of the algorithm. Then the probability that $e$ is available in the next round is at least
%\begin{align*}
%e^{-2 r_i} \cdot \frac{1-x_e/p}{1-x_e}+ (r_i - x_u^i) (1-\frac{e^{-r_i}-1}{r_i}) \,.
%\end{align*}
%
%\textcolor{red}{to Mahsa: the proof for the first part is in the jamboard (stochastic matching) page 10
%Proof of the second part is in the PDF that I sent you.
%}
%\end{lemma}
%
%\begin{proof}
%Consider an edge $e$ that is available at the round $i$ of the algorithm. Based on the algorithm, this edge is available in the next round, if both its end-points are unmatched and it is not queried in round $i$. Thus, we have:
%
%\begin{align}\Pr[e = (v, u) \text{ is available in round } i] & = \Pr[ u \notin M_i  \;\&\;  v\notin M_i \;\&\;  e \text{ is not queried}] \\ & =\end{align}
%
%First of all, observe that 
%\end{proof}
%
%
%
%
%\begin{lemma} \mdcomment{todo}
%Consider a random edge $e$ that is available in round $i$ of the algorithm. We have $$\Pr[e\notin M_i \;|\; e \text{ queried and realized in round }i] \geq e^{x_e-r_i}.$$
%\end{lemma}
%
%
%\begin{lemma}\mdcomment{todo}
%For any $i>1$ and any vertex $u\in V_2$, who is available in round $i$ of the algorithm, w.h.p. we have  $\sum_{e\in E_u} x_e \leq re^{-r} + o(p)$ where $E_u$ is the set of available  edges connected to vertex $u$ in round $i$.
%\end{lemma}



